Tropicalizing abelian covers of algebraic curves

In this thesis, we study the Berkovich skeleton of an algebraic curve over a discretely valued field $K$. We do this using coverings $C\rightarrow{\mathbb{P}^{1}}$ of the projective line. To study these coverings, we take the Galois closure of the corresponding injection of function fields $K(\mathbb{P}^{1})\rightarrow{K(C)}$, giving a Galois morphism $\overline{C}\rightarrow{\mathbb{P}^{1}}$. A theorem by Liu and Lorenzini tells us how to associate to this morphism a Galois morphism of semistable models $\mathcal{C}\rightarrow{\mathcal{D}}$. That is, we make the branch locus disjoint in the special fiber of $\mathcal{D}$ and remove any vertical ramification on the components of $\mathcal{D}_{s}$. This morphism $\mathcal{C}\rightarrow{\mathcal{D}}$ then gives rise to a morphism of intersection graphs $\Sigma(\mathcal{C})\rightarrow{\Sigma(\mathcal{D})}$. Our goal is to reconstruct $\Sigma(\mathcal{C})$ from $\Sigma(\mathcal{D})$ and we will do this by giving a set of covering and twisting data. These then give algorithms for finding the Berkovich skeleton of a curve $C$ whenever that curve has a morphism $\overline{C}\rightarrow{\mathbb{P}^{1}}$ with a solvable Galois group. In particular, this gives an algorithm for finding the Berkovich skeleton of any genus three curve. These coverings also give a new proof of a classical result on the semistable reduction type of an elliptic curve, saying that an elliptic curve has potential good reduction if and only if the valuation of the $j$-invariant is positive.

==> Abstract.tex <==
In this thesis, we study the Berkovich skeleton of an algebraic curve over a discretely valued field $K$. We do this using coverings $C\rightarrow{\mathbb{P}^{1}}$ of the projective line. To study these coverings, we take the Galois closure of the corresponding injection of function fields $K(\mathbb{P}^{1})\rightarrow{K(C)}$, giving a Galois morphism $\overline{C}\rightarrow{\mathbb{P}^{1}}$. A theorem by Liu and Lorenzini tells us how to associate to this morphism a Galois morphism of semistable models $\mathcal{C}\rightarrow{\mathcal{D}}$. That is, we make the branch locus disjoint in the special fiber of $\mathcal{D}$ and remove any vertical ramification on the components of $\mathcal{D}_{s}$.  % associated to this Galois morphism. %$C\rightarrow{\mathbb{P}^{1}}$. 
This morphism $\mathcal{C}\rightarrow{\mathcal{D}}$ then gives rise to a morphism of intersection graphs $\Sigma(\mathcal{C})\rightarrow{\Sigma(\mathcal{D})}$. Our goal is to reconstruct $\Sigma(\mathcal{C})$ from $\Sigma(\mathcal{D})$ and % and some additional data given by the covering $C\rightarrow{D}$.
we will do this by giving a set of covering and twisting data. % for the covering $C\rightarrow{D}$. %assigning covering and twisting data to the covering $C\rightarrow{D}$. 
These then give algorithms for finding the Berkovich skeleton of a curve $C$ whenever that curve has a morphism $\overline{C}\rightarrow{\mathbb{P}^{1}}$ with a solvable Galois group. In particular, this gives an algorithm for finding the Berkovich skeleton of any genus three curve. These coverings also give a new proof of a classical result on the semistable reduction type of an elliptic curve, saying that an elliptic curve has potential good reduction if and only if the valuation of the $j$-invariant is positive.   %This then gives explicit algorithms for finding the Berkovich  %The covering data is the local degree around every vertex and edge of $\Sigma(\mathcal{D})$. We will give explicit formulae for these in terms of decomposition and inertia groups. The twisting data consists  


 %The covering data consists of   %The covering data consists 

%We give explicit formulae for the decomposition and inertia groups of the intersection points and components in $\mathcal{C}$. To completely    

 % These coverings are quite often not Galois an

==> Acknowledgements.tex <==
The author would like to thank his supervisor Professor Eva Maria Feichtner and second referee Associate Professor Joseph Rabinoff for making this thesis possible. Furthermore, the author would like to thank Professor Bernd Sturmfels for his enthusiasm and encouragement throughout the project. The author would also like to thank Madeline Brandt, dr. Martin Ulirsch and Professor Matt Baker for reading through early versions of this thesis and for their helpful remarks. 

This thesis could not have been made without the help of the author's family and friends during this project, for which the author is extremely grateful. The author would also like to thank the Max-Planck Institute for Mathematics in the Sciences in Leipzig for their hospitality during the summer, where he wrote a paper with Madeline Brandt about tropical superelliptic curves. Furthermore, the author would like to thank the Technische Universit\"{a}t Berlin and the Universi\"{a}t Regensburg for their hospitality during two conferences on tropical and non-archimedean geometry, where the author gave two talks on this thesis. 

 %For a lack of       
